Testing Closeness of Multivariate Distributions via Ramsey Theory

We investigate the statistical task of closeness (or equivalence) testing for multidimensional distributions. Specifically, given sample access to two unknown distributions $\mathbf p, \mathbf q$ on $\mathbb R^d$, we want to distinguish between the case that $\mathbf p=\mathbf q$ versus $\|\mathbf p-\mathbf q\|_{A_k} > \epsilon$, where $\|\mathbf p-\mathbf q\|_{A_k}$ denotes the generalized ${A}_k$ distance between $\mathbf p$ and $\mathbf q$ -- measuring the maximum discrepancy between the distributions over any collection of $k$ disjoint, axis-aligned rectangles. Our main result is the first closeness tester for this problem with {\em sub-learning} sample complexity in any fixed dimension and a nearly-matching sample complexity lower bound. In more detail, we provide a computationally efficient closeness tester with sample complexity $O\left((k^{6/7}/ \mathrm{poly}_d(\epsilon)) \log^d(k)\right)$. On the lower bound side, we establish a qualitatively matching sample complexity lower bound of $\Omega(k^{6/7}/\mathrm{poly}(\epsilon))$, even for $d=2$. These sample complexity bounds are surprising because the sample complexity of the problem in the univariate setting is $\Theta(k^{4/5}/\mathrm{poly}(\epsilon))$. This has the interesting consequence that the jump from one to two dimensions leads to a substantial increase in sample complexity, while increases beyond that do not. As a corollary of our general $A_k$ tester, we obtain $d_{\mathrm TV}$-closeness testers for pairs of $k$-histograms on $\mathbb R^d$ over a common unknown partition, and pairs of uniform distributions supported on the union of $k$ unknown disjoint axis-aligned rectangles. Both our algorithm and our lower bound make essential use of tools from Ramsey theory.

==> old-proof.tex <==
The three samples will yield the outcome if there exists a permutation $\pi \in S_3$ such that
$
\ell_{\pi_i} = \beta_i  \, ,
x_{\pi_1} < x_{\pi_2} < x_{\pi_3} \, ,
y_{\pi_1} < y_{\pi_2} < y_{\pi_3}.
$
Therefore, we can rewrite the first term as
$$
\sum_{ \pi \in S_3 }
\Pr \lp[  \ell_{\pi_i} = \beta_i  \, ,
x_{\pi_1} < x_{\pi_2} < x_{\pi_3} \, ,
y_{\pi_1} < y_{\pi_2} < y_{\pi_3}
\rp].
$$
To simplify the expression, we can first take the expectation over $\ell_{\pi_2}, x_{\pi_2}, y_{\pi_2}$.
Condition on the value of $x_{\pi_2}, y_{\pi_2}$, the events $\lp \{ \ell_{\pi_3} =\beta_3, x_{\pi_3} > x_{\pi_2}, y_{\pi_3} > y_{\pi_2} \rp\}$ and $\lp \{ \ell_{\pi_1} = \beta_1, x_{\pi_1} < x_{\pi_2}, y_{\pi_1} < y_{\pi_2} \rp\}$ then becomes independent. 
Hence, we can further rewrite the expression as
\begin{align*}
% &\Pr [  \sigma_{\No} = (1,2,3),  \ell_{\No} = (\beta_1, \beta_2, \beta_3) | \p_{\No} = \t, \q_{\No} = \r] \\
% &=
\sum_{\pi \in S_3}
\E_{ x_{\pi_2}, y_{\pi_2}, \ell_{\pi_2} }
% \int_{a_2, b_2} \lp( \beta_2 \cdot \t(a_2, b_2)
% + (1 - \beta_2) \cdot \r(a_2, b_2) \rp)
\Big[ \mathbbm 1 \{ \ell_{\pi_2} = \beta_2 \}
\cdot \Pr[ \ell_{ \pi_1 } = \beta_1, x_{ \pi_1 } < a_2, y_{\pi_2} < b_2]
 \cdot \Pr[ \ell_{ \pi_3 } = \beta_3, x_{ \pi_3 } > a_2, y_{\pi_3} > b_2] \Big].
% \Bigg[
% % \int_{a_2, b_2} 
% % \Pr [ x_{\pi_2} = a_2, y_{\pi_2} = b_2 ] 
% \Pr [  \ell_{\pi_2} = \beta_2 | x_{\pi_2}, y_{\pi_2} ]
% \cdot 
% \E_{ x_{\pi_3}, y_{\pi_3} }
% \bigg[
% \Pr [ \ell_{\pi_3} = \beta_3 | x_{\pi_3}, y_{\pi_3}] 
% \mathbbm 1 \lp \{ x_{\pi_3} > x_{\pi_2}, y_{\pi_3} > y_{\pi_2} \rp\}
% \bigg]
% \\
% & \cdot 
% \E_{ x_{\pi_1}, y_{\pi_1} }
% \bigg[
% \Pr [ \ell_{\pi_1} = \beta_1  | x_{\pi_1} , y_{\pi_1} ] 
% \mathbbm 1 \lp \{x_{\pi_1} < x_{\pi_2}, y_{\pi_1} < y_{\pi_2} \rp \}
% \bigg]
% \Bigg].
% \intd a_2  \, \intd b_2
\end{align*}
% From here, we will break into the cases depending on whether $\p_{\No}$ is $\t$ or $\r$. 
% Case I ($\p_{\No} = \t$ and $\q_{\No} = \r$). 
We will then analyze the joint distribution of the sample $(x_i, y_i, \ell_i)$.
Notice that the density function depends on whether we are sampling from 
$D( \t, \r, 3 )$ or $D( \r, \t, 3 )$.
For now, we focus on the case that $T_{\No}$ comes from $D( \t, \r, 3 )$.
Then, if $\ell_i = 1$, $(x_i, y_i)$ comes from the distribution $\t$; otherwise, $(x_i, y_i)$ comes from the distribution $\r$.
We can then conclude that the probability density of the sample taking the value $(a, b, \beta)$ should be
$\beta \cdot \t(a, b) + (1 - \beta) \cdot \r(a,b) $.
Using the fact, we can further simplify the expression as (under the assumption $T_{\No} \sim D(\t, \r, 3)$)
\begin{align*}
& \sum_{\pi \in S_3}
\int_{ a_2, b_2  } 
\big( 
\beta_2 \cdot \t(a_2, b_2) 
+ (1 - \beta_2) \cdot 
\r (a_2, b_2)
\big)
\\
&\cdot 
\lp( \int_{ a_3 > a_2, b_3 > b_2 }
 \t(a_3, b_3) \beta_3 + (1 - \beta_3) \r(a_3, b_3)
 \, \intd a_3 \, \intd b_3 \rp)  \\
& \cdot 
\lp( 
\int_{ a_1 < a_2, b_1 > b_2 }
\t(a_1, b_1) \beta_1 + (1 - \beta_1) \r (a_1, b_1) 
 \, \intd a_1 \, \intd b_1
 \rp) \, \intd a_2 \, \intd b_2
\end{align*}
Notice that the expressions for different $\pi \in S_3$ are identical. Hence, we can from here drop the summation $\pi \in S_3$ and multiply the inner expression by $3!=6$ instead.

Now, we will use \Cref{clm:equal-mass}, which immediately gives us
$$
 \int_{a' > a, b' > b} \r(a', b') \intd a' \, \intd b'  = \int_{a' > a, b' > b} \t(a', b') \intd a' \, \intd b'  \, ,$$
$$
  \int_{a' < a, b' < b} \r(a', b')  \intd a' \, \intd b'= \int_{a' < a, b' < b} \t(a', b') \intd a' \, \intd b'.
$$
For convenience, we denote the first quantity as $Q_1(a,b)$ and the second quantity as $Q_2(a,b)$.
We can then further simplify the expression and cancel the terms involving $\beta_1, \beta_3$.
\begin{align} \label{eq:half-case}
&
% \sum_{\pi \in S_3}
6 \cdot \int_{ a_2, b_2  } 
\lp( 
\beta_2 \cdot 
\t(a_2, b_2)
+ (1 - \beta_2) \cdot \r(a_2, b_2)
\rp)
\cdot 
Q_1(a_2, b_2)
\cdot 
Q_2(a_2, b_2)
\intd a_2 \intd b_2
.
% \intd a_2 \intd b_2
% \\ 
% +
% &
% % \sum_{\pi \in S_3}
% 3 \cdot \int_{ a_2, b_2  } 
% \lp( 
% \beta_2 \cdot \q_{\No}(a_2, b_2) + (1 - \beta_2) \cdot \t(a_2, b_2)
% \rp)
% \cdot 
% Q_1(a_2, b_2)
% \cdot 
% Q_2(a_2, b_2)
% \intd a_2 \intd b_2.
\end{align}
Notice that Equation~\eqref{eq:half-case} is the probability of obtaining the patterns $ \sigma_{\No} = (1,2,3),  \ell_{\No} = (\beta_1, \beta_2, \beta_3)$ \emph{condition on} that $(\sigma_{\No}, \ell_{\No})$ comes from $\mathcal D(\t, \r, 3)$. 
By symmetry, the probability for the case that $(\sigma_{\No}, \ell_{\No})$ comes from $\mathcal D(\r, \t, 3)$ has almost the same expression except that we need to exchange $\r$ and $\t$.
Thus, in total, we have
\begin{align*}
&\Pr [ \sigma_{\No} = (1,2,3),  \ell_{\No} = (\beta_1, \beta_2, \beta_3) ]  \\
&= 
3 \cdot \int_{ a_2, b_2  } 
\lp( 
\beta_2 \cdot \lp(\t (a_2, b_2) + \r (a_2, b_2) \rp)
+ (1 - \beta_2) \cdot \lp(\t(a_2, b_2) + \r(a_2, b_2)\rp)
\rp)
\cdot 
Q_1(a_2, b_2)
\cdot 
Q_2(a_2, b_2) \\
&=
3 \cdot \int_{ a_2, b_2  } 
\big( 
\r(a_2, b_2) + 
\t(a_2, b_2)
\big)
\cdot  Q_1(a_2, b_2)
\cdot Q_2(a_2, b_2)  \intd a_2 \intd b_2.
\end{align*}
This shows the probability $\Pr [ \sigma_{\No} = (1,2,3),  \ell_{\No} = (\beta_1, \beta_2, \beta_3) ]$ is indeed independent of $(\beta_1, \beta_2, \beta_3)$, implying the distribution of $\ell_{\No}$ conditioned on $\sigma_{\No} = (1,2,3)$ is uniform.

% ---------------------------

$\Pr [ \sigma_{\No} \in  \{ (1,3,2), (1,2,3) \}, \ell_{\No} = (\beta_1, \beta_2, \beta_3) ]$ is independent of $\beta_i$. Notice that the event $\sigma_{\No} \in  \{ (1,3,2), (1,2,3) \}, \ell_{\No} = (\beta_1, \beta_2, \beta_3)$ happens if and only if there exists a permutation $\pi$ such that
$$
\ell_{\pi_i} = \beta_i  \, ,
x_{\pi_1} < \min\lp( x_{\pi_2}, x_{\pi_3} \rp) \, ,
y_{\pi_1} < \min \lp( y_{\pi_2}, y_{\pi_3} \rp).
$$
Hence, we can write
\begin{align*}
&\Pr [ \sigma_{\No} \in \{ (1,2,3), (1,3,2) \}, \ell_{\No} = (\beta_1, \beta_2, \beta_3) ] \\
&=
\sum_{\pi \in S_3}
\E_{x_{\pi_1}, y_{\pi_1}, \ell_{\pi_1}} \Bigg[
\mathbbm 1 \{ \ell_{\pi_1} = \beta_1 \} \cdot \prod_{j= 2, 3} 
\Pr[ x_{\pi_j} > x_{\pi_1 }, y_{\pi_j} > y_{\pi_1}, \beta_j = \ell_{\pi_j} ]
% \E_{ x_{\pi_j}, y_{\pi_j} }
% \bigg [
% \Pr [ \beta_j = \ell_{\pi_j} | x_{\pi_j}, y_{\pi_j} ]
% \mathbbm 1 \lp \{
% x_{\pi_j} > x_{\pi_1},
% y_{\pi_j} > y_{\pi_1}
% \rp \}
% \bigg]
\Bigg]
\end{align*}
From there, one can show via similar techniques as the ones used in the analysis for $\sigma_{\No} = (1,2,3)$ that the above probability is equal to
\begin{align*}
&\Pr [ \sigma_{\No} \in \{ (1,2,3), (1,3,2) \}, \ell_{\No} = (\beta_1, \beta_2, \beta_3) ] \\
% &=
% \Theta(1) \cdot 
% \int_{a_1, b_1} 
% \Pr [ x_{\pi_1} = a_1, y_{\pi_2} = b_1 ] 
% \cdot  
% \Pr [ \beta_1 = \ell_{\pi_1} | x_{\pi_1} = a_1, y_{\pi_1} = b_1 ]
% \lp( \beta_1 \cdot \t(a_1, b_1) + (1 - \beta_1) \cdot \r(a_1, b_1) \rp)
% \cdot  \lp( \int_{ a' > a_1, b' > b_1 }
% \t(a', b') \rp)^2 \\
&=
3 \cdot 
 \int_{a_1, b_1} 
 \lp( \r(a_1, b_1) 
 + \t(a_1, b_1) \rp)
\cdot  \lp( Q_1(a_2, b_2)  \rp)^2
\intd a_1 \intd b_1.
\end{align*}

==> tester.tex <==
\subsection{The Tester} \label{sec:tester}
\snote{A reviewer wants the algorithm to appear at the beginning of Section 2.2. It is probably a bit hard to implement this organization strategy literally as the algorithm requires multiple non-trivial definitions. We can probably give the definitions and the algorithm and defer the proof to be after the algorithm.}
We begin with an assumption that helps simplify our analysis: the cumulative
density function of each coordinate of
$\p$ or of $\q$ is continuous. We will eventually remove the assumption in the proof of our main theorem.


Suppose that $\snorm{\Ak}{\p - \q} \geq \eps$. We have that there exist $k$ disjoint axis-aligned rectangles $R_1, R_2, \cdots, R_k \subseteq \R^d$ such that $\sum_i \abs{\p( R_i ) - \q(R_i)} \geq \eps$. 
However, as we have shown in Section~\ref{sec:discrepancy}, if two points happen to fall in some rectangle $R_i$, the rectangles formed by them will capture a non-trivial fraction of discrepancy in $R_i$.
For this reason, instead of trying to identify the ``optimal'' rectangles $R_i$, we will instead restrict our attention to rectangles lying on the \emph{sample point grid} defined below.
\begin{definition}[Sample Point Grid] \label{def:grid}
Let $S = \{  x^{(1)}, \cdots, x^{(m)} \} \subset \R^d$ 
be a set of sample points such that no two points overlap in any of their coordinates, i.e. $x^{(i)}_{\ell} \neq x^{(j)}_{\ell}$ for any $i \neq j \in [m]$ and $\ell \in [d]$.
The sample point grid {$G_S$} with respect to the points $S$ is the set of all possible points $z \in \R^d$ such that the $i$-th coordinate $z_i$ is chosen from the set $\{ x^{(1)}_i, \cdots, x^{(m)}_i \}$. 
 % This gives us a grid $G$ consisting of $m^d$ grid points. 
Given an axis-aligned rectangle $R$, we say that $R$ is a grid-aligned rectangle with respect to $G_S$ if all its vertices are grid points from $G_S$.
\end{definition}
Let $G_S$ be a sample grid with respect to a set of sufficiently many \text{i.i.d.} samples from $(\p + \q)/2$.
We first argue that, with decently high probability,
there exist $O(k)$ many rectangles aligned with $G_S$ that capture enough discrepancy between $\p, \q$.
\begin{lemma}
\label{lem:grid-point-discrepancy}
Let $\alpha_d>0$ be the number from \Cref{lem:rectangle-discrepancy}.
Let $\p, \q$ be distributions over $\R^d$ satisfying
$\snorm{\Ak}{\p - \q} > \eps$.
{
Let $S$ be a set of $\Poi(m)$ i.i.d.\ samples from $(\p + \q)/2$, where $k > m \geq C \;  \sqrt{k} / (\eps/4)^{2 \alpha_d}$ for some sufficiently large constant $C$, and
$G_S$ be the sample point grid constructed with these points.
With probability at least $9/10$, there exist $ k' \leq 3k$ disjoint grid-aligned rectangles $\tilde R_1, \cdots, \tilde R_{k'}$ with respect to $G_S$} satisfying that
(i) $ \p(\tilde R_i) + \q(\tilde R_i)   \leq O(1/k)$ for all $i \in [k']$, and
(ii) $\sum_{i=1}^{k'} \lp(\p( \tilde R_i) - \q(\tilde R_i)\rp)^2 \geq \Omega( (\eps/4)^{2 \alpha_d} \; m^2 / k^3 )$.
\end{lemma}
\begin{proof}
Let $R_1, \cdots, R_k$ be the $k$ axis aligned rectangles which realizes the $\Ak$ distance between $\p, \q$. Namely, it holds
$$
\snorm{\Ak}{\p - \q} = \sum_{i=1}^k \abs{ \p(R_i) - \q(R) }.
$$
For convenience, for each rectangle $R_i$, we will denote $v_i \eqdef ( \p(R_i) + \q(R_i) ), \eps_i \eqdef \abs{ \p(R_i) - \q(R_i) } / v_i$.
We first perform some preliminary simplifications to make sure we have
$v_i = O(1/k)$ and $\eps_i \geq \eps / 4$.
Given $ v_i > 1/k$, we can sub-divide $R_i$ into $ \floor{v_i \; k}$ sub-rectangles along the first coordinate evenly according to {the cumulative density function of the first coordinate of $(\p + \q)/2$.}
% As a result, 
% each of the sub-rectangle will have mass upper bounded by $2/k$ and we increase the number of rectangles by at most $2k$.
Next, we discard any rectangles $R_i$ such that $\eps_i < \eps / 4$.
Then, we lose at most $\sum_{i} (\p(R_i) + \q(R_i)) \; \eps/4 \leq \eps/2$ discrepancy. 
In summary, after these operations, we will have $\tilde k \leq 3k$ rectangles $R_1, \cdots, R_{\tilde k}$ such that for each rectangle $R_i$, we have $v_i \leq 1/k$, $\eps_i \geq \eps/4$ and 
$\sum_{i=1}^{\tilde k} v_i \eps_i \geq \eps/2$.


We define the random variable $Y_i$ as follows:
if exactly two samples $x,y$ fall in $R_i$, then 
$Y_i = \lp( \p(R_{x,y}) - \q(R_{x,y}) \rp)^2 $; otherwise, $Y_i = 0$.
{Based on the definition, we can always find 
some disjoint grid-aligned rectangles $\tilde R_1, \cdots, \tilde R_{k'}$, each a subset of some $R_j$, satisfying $\sum_{i=1}^{k'} \lp( \p(\tilde R_i) - \q(\tilde R_i) \rp)^2 = \sum_{i=1}^{k'} Y_i$.
}
Notice that since each $\tilde R_i$ is a subset of some $R_j$, it is guaranteed that $
\p ( \tilde R_i)
+ \q ( \tilde R_i) 
\leq 
O(1/k)
$ for each $i \in [k']$.
Our lemma follows if we can show $\sum_{i=1}^{\tilde k} Y_i \geq
\Omega \lp( (\eps/4)^{2 \alpha_d } \; m^2 / k^3 \rp)
$ holds with probability at least $9/10$.

Consider the event $E_i$ defined as that exactly two sample points fall inside $R_i$.
It is easy to see that
$$
\Pr[ E_i] = 
\Pr \lp[\Poi(m \; v_i / 2) = 2  \rp]
= \Theta(1) \; (m \; v_i)^2.
$$
Conditioned on $E_i$, $Y_i$ is exactly $\lp( \p(R_{x,y}) - \q(R_{x,y}) \rp)^2$ where $x,y$ are two random points from $ \frac{1}{2} (\p + \q)_{|R_i}$.
By our preliminary simplification, we have
$\abs{\p(R_i) - \q(R_i)} \geq \eps/4 \; \lp(\p(R_i) + \q(R_i) \rp)$.
Hence, applying \Cref{lem:rectangle-discrepancy} then gives us
$$
\underset{{ x,y \sim \frac{1}{2} (\p + \q)_{|R_i} }} \E \lp[ \abs{\p(R_{x,y}) - \q(R_{x,y})} \rp]
\geq 
\eps_i^{\alpha_d} v_i.
$$
Combining this with Jensen's inequality then gives that
$$
\underset{{ x,y \sim \frac{1}{2} (\p + \q)_{|R_i} }} \E \lp[ \lp(\p(R_{x,y}) - \q(R_{x,y}) \rp)^2 \rp]
\geq 
\lp( \underset{{ x,y \sim \frac{1}{2} (\p + \q)_{|R_i} }} \E \lp[ \abs{\p(R_{x,y}) - \q(R_{x,y})} \rp] \rp)^2
\geq
\eps_i^{2\alpha_d} v_i^2.
$$
Since $Y_i$ conditioned on $E_i$ is distributed exactly like $\lp( \p(R_{x,y}) - \q(R_{x,y}) \rp)^2$ and is always non-negative, we thus have
\begin{align} \label{eq:single-yi-bound}
\E[Y_i] 
\geq
\E[Y_i | E_i] \; \Pr[E_i]
\geq \Omega(1) \; (m \; v_i)^2 \; \eps_i^{ 2  \alpha_d }  v_i^2
\geq \Omega(1) \; \eps_i^{ 2  \alpha_d }
\; m^2 \; v_i^4.    
\end{align}
Summing over all $Y_i$, we thus have
\begin{align*}
\sum_{i=1}^{k'} \E[Y_i] 
\geq 
\Omega(1) \;
\sum_{i=1}^{k'}  \eps_i^{ 2  \alpha_d -4 }
\; m^2 \; (v_i \eps_i) ^4
\geq 
\Omega(m^2) \; (\eps/4)^{ 2  \alpha_d -4 }
\sum_{i=1}^{k'}  (v_i \eps_i) ^4
\geq 
\Omega(m^2) \; (\eps/4)^{ 2  \alpha_d } / k^3 \, ,
\end{align*}
where in the first inequality we apply \Cref{eq:single-yi-bound}, in the second inequality we lower bound $\eps_i$ by $\eps/4$, in the third inequality we use the fact that $\sum_{i=1}^{b} a_i^4$ subject to $\sum_i a_i = A$, $a_i \geq 0$ is minimized at $a_i = A/b$.


% and the axis-aligned rectangle $R_{x,y}$ satisfies $ \abs{ \p(R_{x,y}) - \q(R_{x,y}) }  \geq \eps^{ \alpha_d } \; \lp( \p(R_i) + \q(R_i) \rp)$.
% As a result of Poissonization, the events $E_i$ for $i \in [k]$ are independent of each other. 
% Moreover, if $E_i$ happens, we then have $Y_i \geq \alpha_{d, \eps}^2 v_i^2$.
% we know there is a rectangle $R \subseteq U_i$ satisfying
% (i) $\p(R) + \q(R) \leq \p(U) + \q(U) \leq 2/k$.
% (ii) $\abs{\p(R) - \q(R)}^2 \geq  \alpha_{d,\eps}^2 \; v_i^2$.
% We first lower bound the probability that $E_i$ happens, which would then give us a lower bound of $\E[Y_i]$.
% In particular, condition on the event that two samples $x,y$ all in $U_i$, by Lemma \ref{lem:rectangle-discrepancy}, we have that with probability at least $\alpha_{d, \eps}$, 
% $$ \abs{\p(R_{x,y}) - \q(R_{x,y})} \geq \alpha_{d, \eps} \; ( \p(U_i) + \q(U_i) )
% .$$
% Hence, 
% $$
% \Pr[E_i] \geq \Poi( m \; v_i/2, 2) \; \alpha_{d, \eps} \geq \Omega(1) \; \alpha_{d, \eps} \; (m \; v_i)^2.
% $$
% On the other hand, $E_i$ only happens if two samples fall in $U_i$, which easily gives $\Pr[E_i] \leq O( m^2 v_i^2 )$.
On the other hand, since $Y_i$ is defined to be non-zero only when there are two points falling in $Y_i$ and takes value at most $v_i^2$, we have 
$
\Var[Y_i] \leq \Pr[ E_i ] \; v_i^4
= O(1)  \; m^2 \; v_i^6.
$
Furthermore, since each $Y_i$ are independently distributed, 
we have
\begin{align*}
    \Var \lp[ \sum_{i=1}^{k'} Y_i \rp]
    = \sum_{i=1}^{k'}
    \Var[ Y_i ]
    \leq 
    O(1)  \; m^2  \sum_{i=1}^{k'} v_i^6
    \leq O( m^2 / k^5 ) \, ,
\end{align*}
where in the last inequality we use  $v_i \leq O(1/k)$.
% \begin{align*}
% \E \lp[ \sum_{i=1}^{k}  Y_i \rp] &\geq 
% \Omega(1) \; \eps^{2 \alpha_d}  \; m^2 \; \sum_{i=1}^k v_i^4 \, , \\
% \Var \lp[ \sum_{i=1}^{k} Y_i \rp] &\leq O(1) \; m^2 \; \sum_{i=1}^k v_i^6.
% \end{align*}
We then have 
$ 
 \Var[ \sum_{i=1}^{k'} Y_i]  \leq 1/20 \cdot
\lp(  
\E \lp[ \sum_{i=1}^{k'} Y_i \rp] \rp)^2
$
as long as $m \geq C \;  \sqrt{k} / (\eps/4)^{2 \alpha_d}$ for some sufficiently large constant $C$. Then, by Chebyshev's inequality, it follows
$$
\Pr \lp[ 
\sum_{i=1}^k Y_i \geq \Omega( (\eps/4)^{2 \alpha_d} \; m^2/k^3 )
\rp]
\geq 9/ 10.
$$
% Since $v_i = O(1/k)$ and $\sum_{i} v_i \leq 1$, it is easy to see that $ \sum_{i=1}^k v_i^4 \geq O \lp( 1/k^3 \rp)$.
This then conclude the proof of \Cref{lem:grid-point-discrepancy}.
\end{proof}
\Cref{lem:grid-point-discrepancy} states that there exist $k$ grid-aligned rectangles such that they capture at least $\Omega(m^2/k^3)$ discrepancy between $\p, \q$ for constant $d, \eps$.
A naive tester may then do the following: Choose a set of $k$ disjoint rectangles aligned with the sample point grid and then perform closeness testing between the reduced distributions of $\p, \q$ on the chosen rectangles.
Then, if we are lucky, the chosen rectangles will capture enough discrepancy between $\p, \q$ and a standard closeness tester suffices.
Yet, there are many different ways to choose $k$ disjoint grid-aligned rectangles. 
The tester would be clearly inefficient if we were to try all possible combinations.
To circumvent the issue, we 
will consider a carefully chosen family of all grid-aligned rectangles with respect to the sample point grid such that any grid-aligned rectangles can be decomposed into the union of a small number of rectangles from the family. This leads us to the concept of \emph{Grid Covering}, which is based on 
the idea of \emph{Good Oblivious Covering} (Definition 2 from \cite{diakonikolas2019testing}).
\begin{definition}[Grid Covering] \label{def:grid-cover}
{Let $S$ be a set of $(m+1)$ points in $\R^d$ and $G_S$ be the corresponding sample point grid.} 
the grid covering is a family of rectangles algined with the sample point grid, which we denote by $\mathcal F(G_S)$, satisfying the following:
\begin{itemize}
    \item Any rectangle aligned with the grid can be represented as the union of $2^d \; \log^d m$ disjoint rectangles from $\mathcal F(G_S)$.
    \item Any point in $\R^d$ is included in exactly $\log^d m$ rectangles.
\end{itemize}
\end{definition}
With a construction similar to that in \cite{diakonikolas2019testing}, we show that a Grid Covering indeed exists.
\begin{lemma}
Let $m$ be a power of $2$, {$S$ be a set of $(m+1)$ points from $\R^d$ and $G_S$ be the corresponding sample point grid.}
Then, there exists a grid covering $\mathcal F(G_S)$.
\end{lemma}
\begin{proof}
For each coordinate $j \in [d]$, let $x^{(1)}_j, \cdots, x^{(m+1)}_j$ be the possible values of the grid points sorted in increasing order.
We will denote these numbers as the ``grid values''.
For each $i \in  [\log m]$, we will define $\mathcal I_{j, i}$ as the partition of the interval $[x^{(1)}_j, x^{(m)}_j]$ into $2^i$ many intervals such that each sub-interval in the partition spans across an equal number of grid values.
Then, the rectangles in $\mathcal F(G_S)$ are those of the following form: for $j \in [d]$, an interval $I_j \in \bigcup_i \mathcal I_{j, i}$ is chosen and the rectangle is simply the product of the $d$ selected intervals $I_j$.

Then it is easy to see that for any value $ z \in [ x^{(1)}_j, x^{(m+1)}_j ] $, $z$ is within exactly $\log m$ intervals from $\bigcup_i \mathcal I_{j, i}$ (one interval from each partition). As a result, any point in $\R^d$ is within at most $ \log^d m $ rectangles from $\mathcal F(G_S)$.

Let $R$ be a grid aligned rectangle that is the product of the intervals $I_1, \cdots I_d$. Notice that the interval $I_j$ can be decomposed into at most $2 \; \log m$ intervals from $\bigcup_i \mathcal I_{j, i}$ (at most $2$ intervals from each partition $\mathcal I_{j,i}$). Thus, $R$ can be decomposed into at most $2^d \; \log^d m$ rectangles from $\mathcal F(G_S)$.
\end{proof}
We next consider the \emph{induced distribution} of $\p, \q$ on $\mathcal F(G_S)$.
\begin{definition}[Induced Distribution]
Given $\p$ on $\R^d$ and a family of sets $\mathcal F$ {whose elements are non-empty sets in 
$\R^d$ that are not necessarily disjoint}, the induced distribution $\p^{\mathcal F}$ is defined as 
follows. To take a random sample from $\p^{\mathcal F}$, one first takes a random point $x$ from 
$\p$. {If $x$ does not belong to any set in $\mathcal F$, one returns a special element 
$\emptyset$. Otherwise, 
 one returns a uniform random set $S \in \mathcal F$ such that $x \in S$.}
\end{definition}
% Let $R$ be a rectangle 
% Suppose the grid $G$ captures $\gamma$ discrepancy between $\p, \q$ and 
% $\mathcal F(G_S)$ is its grid covering. Then, it is easy to see that $\snorm{1}{ \p^{\mathcal F(G_S)} - \q^{\mathcal F(G_S)} } \geq \gamma / \log^d m$ since $ \abs{ \p^{\mathcal F(G_S)} (R) - \q^{\mathcal F(G_S)}} (R) \geq \log^{-d} m \; \abs{ \p(R) - \q(R) }$ for any rectangle $R \in \mathcal F(G_S)$.
Notice that for a rectangle $R \in \mathcal F(G_S)$. We have that 
$\p^{\mathcal F(G_S)}(R) = \p(R) / \log^d m$, 
since each point appears in exactly $\log^d m$ rectangles from $\mathcal F(G_S)$. 
This then allows us to show that the $\ell_2$-discrepancy between 
the induced distributions $\p^{\mathcal F(G_S)}, \q^{\mathcal F(G_S)}$ 
must be non-trivial if the grid $G$ satisfies the 
condition in \Cref{lem:grid-point-discrepancy}. 
Specifically, we show:
\begin{lemma} \label{lem:induced-discrepancy}
{Let $m$ be a power of $2$, $S$ be a set of $(m+1)$ points 
from $\R^d$ and $G_S$ be the corresponding sample point grid.}
Moreover, suppose that the conclusion of \Cref{lem:grid-point-discrepancy} is satisfied for $G_S$.
Then there exists a subset of rectangles $H \subset \mathcal F(G_S)$ such that 
(i) $\abs{H} \leq 3k \; 2^d \log^d m$, 
(ii) $\p(R) + \q(R) \leq  O(1/k)$ for all $R \in H$, and 
(iii)
$$\sum_{ R \in H } \lp( \p^{\mathcal F(G_S)}(R) - \q^{\mathcal F(G_S)}(R) \rp)^2 
\geq \Omega(1) \; 
2^{-d} \; \log^{-3d} (k) \; (\eps/4)^{2\alpha_d } \; m^2 / k^3 \;.
$$
\end{lemma}
\begin{proof}
By the guarantees of \Cref{lem:grid-point-discrepancy}, there exists $k' \leq 3k$ many grid-aligned rectangles (with respect to $G$) $R_1, \cdots, R_{k'}$ rectangles satisfying 
$  \p(R_i) + \q(R_i)   \leq O\lp( 1/k \rp)$ for all $i \in [k']$, and
\begin{align} \label{eq:initial-discrepancy}
\sum_{i=1}^{k'} \abs{\p(R_i) - \q(R_i)}^2 \geq \Omega( (\eps/4)^{2 \alpha_d}  \; m^2 / k^3 ).
\end{align}
% Suppose the algorithm does not add any extra points to $S$. The claim follows from \Cref{lem:grid-point-discrepancy}. 
% Now, it is easy to see that $R_1, \cdots, R_k'$ are still grid-aligned rectangles with the extra points. Hence, the claim follows.
% Let $\mathcal F(G_S)$ be a grid-covering.
% Recall that the induced distributions $\p^{\mathcal F(G_S)}, \q^{\mathcal F(G_S)}$ are distributions over rectangles in $\mathcal F(G_S)$. 
% We will show that there exists a set of rectangles $H \subset \mathcal F(G_S)$ with $\abs{H} \leq k \; 2^d \log^d m$ such that
% $ \p^{\mathcal F(G_S)}(R) + \q^{\mathcal F(G_S)}(R)   \leq O\lp( 1/k \rp)$ for $R \in H$ and
% \begin{align} \label{eq:induced-discrepancy}
% \sum_{R \in H} \lp( \p^{\mathcal F(G_S)}(R) - \q^{\mathcal F(G_S)}(R) \rp)^2
% \geq \Omega(1) \; 
% 2^{-d} \; \log^{-2d}(m) \; \eps^{2 \alpha_d}  \; m^2 / k^3.    
% \end{align}
% $\p^{\mathcal F(G_S)}, \q^{\mathcal F(G_S)}$ have non-trivial $\ell_2$ discrepancy.
By the definition of the grid covering, each $R_i$ can be decomposed into at most $2^d \; \log^d(m)$ rectangles from $\mathcal F(G_S)$.
Let $H_i$ be the set of rectangles in $\mathcal F(G_S)$ that $R_i$ is decomposed into.
We will consider $H = \bigcup_i H_i$.
Obviously, $\abs{H} \leq  3k \; 2^d \; \log^d(m)$, which shows (i).
Besides, by the definition of induced distribution, for any rectangle $R \in \mathcal F(G_S)$ we have $\p^{\mathcal F(G_S)}(R) = \log^{-d} (m) \; \p(R) $.
Therefore, for each $R \in H$, it holds 
$ \p^{\mathcal F(G_S)}(R) \leq   \log^{-d} (m) \; O (1/k)$, which shows (ii).

It remains to show (iii). For each $H_i$, we have
\begin{equation*}
% \label{eq:cover-spread}
\sum_{R \in H_i} \lp( \p(R) - \q(R) \rp)^2
\geq 2^{-d} \; \log^{-d}(m) \; \lp( \p(R_i) - \q(R_i) \rp)^2 \, ,
\end{equation*}
since $ \sum_{R \in H_i} \p(R) = \p(R_i) $ (and the same for $\q$) and $\abs{H_i} \leq 2^{d} \; \log^{d} (m) $.
Combining this with the fact that $\p^{\mathcal F(G_S)}(R) = \log^{-d} (m) \; \p(R)$ and 
 Equation~\eqref{eq:initial-discrepancy} then gives claim (iii).
\end{proof}

Unlike the naive testing approach that runs closeness testing on many different pairs of reduced distributions, we can now run closeness tester just on the induced distributions $\p^{\mathcal F(G_S)}, \q^{\mathcal F(G_S)}$.
A technical issue is that the size of the new domain $\mathcal F(G_S)$ is still huge. 
This makes black-box application of any $\ell_1$ closeness tester inefficient.
Instead, we need to exploit the fact that a non-trivial fraction of the discrepancy between them is supported on a small number of elements.
In fact, a similar tester has been developed in \cite{DKN17} (See Lemma 2.5). 
Here, we essentially need to develop an $\ell_2$ version of it. Namely, we want to distinguish between the cases $\p = \q$ versus that a non-trivial amount of $\ell_2$ discrepancy is supported on a few elements that are themselves not too heavy.
In particular, using tools from \cite{DiakonikolasK16}, we show the following.

\begin{lemma}
\label{lem:small-support-l2}
Let $\p, \q$ be two discrete distributions on $[n]$ and $s \in [n]$.
Given $\eps > 0$ and $\Poi(m)$ many \iid samples from $\p, \q$ for $ m = \Theta \lp(  \max \lp( \eps^{-4/3}, \eps^{-2} / \sqrt{s} \rp) \rp)$,
there exists a tester \textsc{ Flatten-Closeness } that can distinguish between the following cases 
with probability at least $9/10$: 
(a) $\p = \q$ versus (b) there exists a set of elements $H$ of size $s$ such that
(i)  $\sum_{i \in H} ( p_i - q_i )^2 \geq \eps^2$
and (ii)  $ \max_{i \in S} (p_i + q_i)/2 \leq 1/s $.
\end{lemma}
\begin{proof}
% \paragraph{Flattening and $\ell_2$-closeness tester.} 
Given a discrete distribution $\p$, 
flattening is the technique of using a set of sample points from $\p$ to subdivide bins 
from the domain that aims at reducing the $\ell_2$-norm of the distribution. 
Formally, the flattening technique yields what was described 
in \cite{DiakonikolasK16} as a \emph{split distribution}.
\begin{definition}
[Definition 2.4 from \cite{DiakonikolasK16}]
Given a distribution $\p$ on $[n]$ and a multiset $S$ of elements of $[n]$, define the \emph{split distribution} $p_S$ on $[n + |S|]$ as follows: For $1 \leq i \leq n$, let $a_i$ denote $1$ plus the number of elements of $S$ that are equal to $i$. Thus, $\sum_{i=1}^n a_i = n + |S|$. We can therefore associate the elements of $[n + |S|]$ to elements of the set $B = \{ (i,j) : i \in [n], 1 \leq j \leq a_i \}$. We now define a distribution $\p_S$ with support $B$, by letting a random sample from $\p_S$ be given by $(i,j)$, where $i$ is drawn randomly from $p$ and $j$ is drawn randomly from $[a_i]$.
\end{definition}

We will use the following basic facts about split distributions.

\begin{fact}
[Fact 2.5 from \cite{DiakonikolasK16}]
Let $p$ and $q$ be probability distributions on $[n]$, and $S$ a given multiset of $[n]$. Then:
(i) We can simulate a sample from $p_S$ or $q_S$ by taking a single sample from $p$ or $q$, respectively. 
(ii) It holds $\snorm{1}{p_S - q_S} = \snorm{1}{p - q}$.
\end{fact}

\begin{lemma}
[Lemma 2.6 from \cite{DiakonikolasK16}]
\label{lem:flatten}
Let $p$ be a distribution on $[n]$. Then: (i) For any multisets $S \in S'$ of $[n]$,
$\snorm{2}{p_{S'}} \leq \snorm{2}{p_{S}}$, and
(ii) If $S$ is obtained by taking $\Poi(m)$ samples from $p$, then $\E \lp[ \snorm{2}{p_S}^2 \rp] \leq 1/m$.
\end{lemma}
% \paragraph{$\ell_2$-Closeness Tester.}
We also rely on the following robust $\ell_2$ closeness tester.
\begin{lemma}
[Proposition 6 from \cite{chan2014optimal} ]
\label{lem:robust-l2}
Let $\p$ and $\q$ be two unknown distributions on $[n]$.
There exists an algorithm that on input $n, \eps > 0$, and $b \geq \max \lp(  \snorm{2}{\p}^2, \snorm{2}{\q}^2 \rp)$ draws $ \Poi(m)$ samples  samples from $\p, \q$ where $m = \sqrt{b} / \eps^2 $, and, with probability $3/4$, distinguishes between the cases $\snorm{2}{\p-\q} = 0$ and
$\snorm{2}{\p-\q} > \eps$.
\end{lemma}

Let $S$ be a multiset of $\Poi(m)$~\iid from $
\lp(\p +\q \rp)/2$ for some $m \leq s / 100$. 
First, we argue that the $\ell_2$ norm between $\p, \q$ will not decrease by too much after flattening by taking advantage of the fact that the $\ell_2$ discrepancy between $\p, \q$ is  supported on a few light elements.
Let $X_i$ be the random variable denoting the number of samples from $S$ falling in the $i$-th element, i.e., $X_i \sim \Poi(m \; \lp( \p_i +\q_i\rp) / 2  )$.
Then, the expected discrepancy restricted to the elements from $E$ after flattening  is at least 
\begin{align*}
\sum_{i \in E} \E \lp[  \frac{\lp(\p_i - \q_i \rp)^2}{ X_i +1 } \rp]
= 
\sum_{i \in E} \lp(\p_i - \q_i \rp)^2 \; (1 - e^{- \lambda_i})/ \lambda_i \, ,
\end{align*}
where we define $\lambda_i \eqdef m \; \lp( \p_i +\q_i\rp) / 2$.
Notice that $(1 - e^{-x})/x$ is a decreasing function with respect to $x$. 
Since $m \leq s / 100$ and $(\p_i +\q_i)/2 \leq s$, it follows that 
$(1 - e^{- \lambda_i})/ \lambda_i$
is bounded below by
$ 1 - e^{ -0.01 } / 0.01 \geq 0.99$.
This then gives us
\begin{align} \label{eq:expect-lower-bound}
\E\lp[ \sum_{i \in E}  \frac{\lp(\p_i - \q_i \rp)^2}{ X_i +1 } \rp]
\geq 
0.99 \sum_{i \in E} \lp( \p_i - \q_i \rp)^2.
\end{align}
On the other hand, the variance is bounded above by
\begin{align*}
\Var \lp[ \sum_{i \in E}  \frac{\lp(\p_i - \q_i \rp)^2}{ X_i +1 } \rp]
&= 
\E \lp[ \lp(\sum_{i \in E}  \frac{\lp(\p_i - \q_i \rp)^2}{ X_i +1 } \rp)^2 \rp]
- \E^2 \lp[ \lp(\sum_{i \in E}  \frac{\lp(\p_i - \q_i \rp)^2}{ X_i +1 } \rp)^2 \rp] \\
&\leq 
 \lp(\sum_{i \in E} \lp( \p_i - \q_i \rp)^2\rp)^2
 - (0.99)^2 \lp(\sum_{i \in E} \lp( \p_i - \q_i \rp)^2 \rp)^2 \, ,
\end{align*}
where in the last inequality we use the fact that $\frac{1}{1 +X_i}$ is at most $1$ and Equation~\eqref{eq:expect-lower-bound}.
This then gives us
\begin{align} \label{eq:var-upper-bound}
    \sqrt{ \Var \lp[ \sum_{i \in E}  \frac{\lp(\p_i - \q_i \rp)^2}{ X_i +1 } \rp] }
    \leq 0.15 \;  \sum_{i \in E} \lp( \p_i - \q_i \rp)^2.
\end{align}
Combining Equations~\eqref{eq:expect-lower-bound} and~\eqref{eq:var-upper-bound} we obtain
\begin{align} \label{eq:good-discrepancy}
    \Pr \lp[ \snorm{2}{ \p_S - \q_S }^2 <  \frac{1}{3} \sum_{i \in E} \lp( \p_i - \q_i \rp)^2  \rp] 
    \leq 1/4
\end{align}
On the other hand, by \Cref{lem:flatten} and Markov's inequality, it holds
\begin{align} \label{eq:good-l2}
    \Pr \lp[ \max \lp( \snorm{2}{ \p }^2, \snorm{2}{ \q }^2 \rp) > 40 / m  \rp]  \leq 1/10.
\end{align}
By the union bound, Equations~\eqref{eq:good-discrepancy} and~\eqref{eq:good-l2} and 
\Cref{lem:robust-l2}, it follow that the $\ell_2$-closeness tester succeeds 
with probability at least $2/3$ if we take  
$m' = C \; \sqrt{ \frac{1}{m} } \; \eps^2$ many samples for a sufficiently large constant $C$. 
Balancing $m$ and $m'$ (with the restriction $m \leq s / 100$ in mind) then gives us that 
the overall tester succeeds with probability at least $2/3$
if it takes $\Poi( m )$ many~\iid samples with 
$$
m = \Theta \lp(  \max \lp( \eps^{-4/3}, \eps^{-2} / \sqrt{s} \rp) \rp) \;.
$$
{This concludes the proof of Lemma~\ref{lem:small-support-l2}.}
\end{proof}
We are now ready to present the detailed testing algorithm and its analysis. 
%using existing tools from \cite{DiakonikolasK16} on $\ell_2$ closeness tester.

\begin{algorithm}[H]
\caption{Multidimensional $\mathcal{A}_k$ Closeness Tester} \label{alg:multi-ak-test}
    \begin{algorithmic}[1]
    \Require  sample access to $\p, \q$ on $\R^d$; failure probability $\delta$; accuracy $\eps$.
    \State Set $m \gets C \; k^{6/7} \; \eps^{ -2 \alpha_d / 3 } \; \log^d(k) \; 2^{d/3}$, 
    where $C'$ is a sufficiently large constant and 
    $\alpha_d$ is the number from \Cref{lem:rectangle-discrepancy}.
    \State Take $\Poi(m)$ samples from $(\p + \q)/2$ and denote the set of samples as $S$.
    \State Add arbitrarily some distinct points to $S$ such that $|S|$ is a power of $2$. \label{line:addpoint}
    \State Construct the grid $G_S$ (\Cref{def:grid}) and the grid covering $\mathcal F(G_S)$ (\Cref{def:grid-cover}).
    % \State Take $\Poi(m)$ samples from $\lp( \p^{\mathcal F(G_S)} +  \q^{\mathcal F(G_S)} \rp) / 2$. Denote the set of samples as $S$ and $ \p^{\mathcal F(G_S)}_S, \q^{\mathcal F(G_S)}_S$ as the corresponding distribution flattened by the samples from $S$.
    \State Run the $\ell_2$-closeness tester from \Cref{lem:small-support-l2} 
    on the induced distributions $\p^{\mathcal F(G_S)}, \q^{\mathcal F(G_S)}$ 
    with accuracy parameter 
    $ \kappa = c \; 2^{-d} \log^{-3d} k \; (\eps/4)^{2 \alpha_d} \; m^2 / k^3 $ 
    for some small enough constant $c$.
    \State Accept if the closeness tester passes; otherwise Reject.
    % (Or normalize it)
    \end{algorithmic}
\end{algorithm}

% \inote{Is the last step of the algorithm correct?}

\begin{proof}[Proof of Upper bound in Theorem~\ref{thm:main-intro}]
We first present the analysis assuming that 
$\p, \q$ are continuous distributions and in the end give a preprocessing step to make sure the algorithm works for general distributions.
Let $F(G_S)$ be defined as in Algorithm~\ref{alg:multi-ak-test}.
If $\p = \q$, we have $\snorm{2}{\p^{\mathcal F(G_S)} - \q^{\mathcal 
F(G)}}^2 = 0 $. Therefore, the tester will accept with probability at least $2/3$.

Next, we consider the case $\snorm{\Ak}{\p - \q} > \eps$.  We claim that with probability at least $9/10$, there exists $k' \leq k$ grid-aligned rectangles (with repect to $G_S$) such that the guarantees of \Cref{lem:grid-point-discrepancy} is satisfied. 
{Without the operation of adding extra points into $S$ in Line~\ref{line:addpoint} of Algorithm~\ref{alg:multi-ak-test}, the claim just follows from \Cref{lem:grid-point-discrepancy}.}
Now, it is easy to see that $R_1, \cdots, R_{k'}$ are still grid-aligned rectangles with the extra points. Hence, the claim follows. 

Condition on the event that the guarantees of \Cref{lem:grid-point-discrepancy} are met. We can then apply \Cref{lem:induced-discrepancy}, which gives us that there exists a set of elements $H \subset \mathcal F(G_S)$ such  that 
(i) $\abs{H} \leq 2^d \log^d m \; k$
(ii) $\p(R) + \q(R) \leq  O(1/k)$ for all $R \in H$ and 
(iii)
$$\sum_{ R \in H } \lp( \p^{\mathcal F(G_S)}(R) - \q^{\mathcal F(G_S)}(R) \rp)^2 
\geq \Omega(1) \; 
2^{-d} \; \log^{-3d} (k) \; (\eps/4)^{2\alpha_d } \; m^2 / k^3.
$$
Then, applying \Cref{lem:small-support-l2} gives that the tester rejects with probability at least $9/10$ given that 
$$
m \geq C  \max \lp(  {\kappa}^{-2/3}
,{\kappa}^{-1} / \sqrt{k}   \ \rp).
$$
where 
$\kappa =  \Theta(1) \;
2^{-d} \; \log^{-3d} (k) \; (\eps/4)^{2\alpha_d } \; m^2 / k^3 $ and $C$ is a large enough constant.
% Substituting the bound $m = k^{6/7} \; \eps^{-c_d'} \; \log^{2d}(k)$ then gives us $m' = C' \; m$ for some sufficiently large constant $C$.
One can verify that
$
m = 
C' \; k^{6/7} \; \eps^{ -2 \alpha_d / 3 } \; \log^d(k) \; 2^{d/3}
$
is enough
where $C'$ is a sufficiently large constant. 
% solving out $m, m'$ then gives us the entire tester succeeds with probability at least $2/3$ if we set
% $$
% m = m' = 
% k^{6/7} \; \eps^{- c_d'} \; \log^{2d}(k)
% $$
% for some number $c_d'$ that depends only on $d$.

Now, let us relax the assumption that the marginal distributions of $\p, \q$ in each coordinate have continuous cumulative density functions.
We begin with the observation that the algorithm's output essentially depends only on the order information of sample points. That is, given two different set of samples $S = \{ x^{(1)}, \cdots, x^{(m)} \}, \tilde S = \{ \tilde x^{(1)}, \cdots  \tilde x^{(m)}\}$ such that the relative orders of $x^{(1)}_j, \cdots, x^{(m)}_j$ and $\tilde x^{(1)}_j, \cdots, \tilde x^{(m)}_j$ are the same for each coordinate $j \in [d]$, the output of the algorithm will always be the same.

Based on the observation, we know the algorithm will enjoy the same guarantee if we give it only the ``rank'' information of the samples. 
 That is, for $j \in [d]$, we sort $x^{(1)}_j, \cdots, x^{(m')}_j$ in increasing order.  
% When there are ties, we break ties uniformly at random.
We will denote by $\pi(j)_i$ as the rank of $x^{(i)}_j$ in the sorted sequence.
Then, for each $i \in [m']$, we replace the original sample with the new sample $\hat x^{(i)}$ defined as $\hat x^{(i)}_j = \pi(j)_i$. 

If $\p, \q$'s marginal distributions are not continuous, we may see multiple samples sharing the same value at some coordinates.
Then, when computing the rank information of the samples, we will break ties uniformly at random.
Now consider the distribution $\p', \q'$ obtained by stretching any point mass of their marginal distributions at any coordinate into an interval.
If the algorithm takes samples from $\p', \q'$ instead, the guarantees are satisfied since $\p', \q'$ are both continuous distributions and $\snorm{\Ak}{\p - \q} = \snorm{\Ak}{\p' - \q'}$. 
On the other hand, the order of samples taken from $\p', \q'$ has the same distribution as the order of samples taken from $\p, \q$ after we break ties uniformly at random. This then concludes the proof.
% Let $F: \R \mapsto [0,1]$ be the cumulative mass function of the marginal distribution of $(\p + \q)/2$ along the first coordinate. If $F$ has a jump-point at $x \in \R$, it means that the marginal distribution must have a point mass at $x$. This means the algorithm may observe multiple sample points from $(\p + \q)/2$ that has their first coordinate being $x$. 
% % Notice that our algorithm depends only on the order information of these points. 
% % What we can do is to simply randomize the order of these ``colliding'' points in the first coordinate. 
% Then, the behavior of the algorithm will be identical to the scenario where the point mass at $x$ is stretched into an interval. 
% Hence, we reduce back to the case where the cumulative mass function is continuous.
\end{proof}

\subsection{
Applications: Closeness Testing of Multivariate Structured Distributions under Total Variation Distance} \label{sec:application}
%In this section, we provide some applications of $\Ak$ closeness testing of multivariate distributions.
The most straightforward application of our general $\Ak$ closeness tester 
is for the problem of testing closeness of multivariate histogram 
distributions --- distributions that are piecewise constant over (the same) \emph{unknown} 
collection of axis-aligned rectangles --- with respect to the total variaton distance.

This follows directly from our main theorem, since for any pair of $k$-histogram distributions
$\p, \q$ with respect to the same set of rectangles,  we have 
$\dtv(\p, \q) = \frac{1}{2} \sum_{i=1}^k \abs{ \p(R_i) - \q(R_i) } = \frac{1}{2} \snorm{\Ak}{\p - \q}$. Formally, we have the following: 

\begin{corollary} \label{cor:md-hist}
Let $\{R_i\}_{i=1}^k$ be an unknown set of axis-aligned rectangles in $\R^d$.
Suppose $\p, \q$ are distributions over $\R^d$ that are piecewise constant over each of $\{R_i\}_{i=1}^k$, i.e., $\p(x) = \p(y)$ for any $x,y \in R_i$ and the same for $\q$.
Then there exists a tester which distinguishes between 
$\p = \q$ and $\dtv(\p, \q) > \eps$ with sample complexity
$
C \; k^{6/7} \; \eps^{ -2 \alpha_d / 3 } \; \log^d(k) \; 2^{d/3}
$, 
where $C$ is a sufficiently large universal constant and $\alpha_d = O(d^2 2^{2^{d+1}})$.
\end{corollary}

A less obvious application is the following. We consider the 
binary hypothesis class $H$ made up of all possible $k$-unions of 
axis-aligned rectangles within the unit cube $[0,1]^d$. Given two 
hypotheses $h_1, h_2 \in H$, we can test whether $h_1$ is 
equivalent to $h_2$ or they are far from each other under the 
uniform distribution over the unit cube $[0,1]^d$.

\begin{corollary}
Let $H$ be the class of all possible $k$-unions of axis-aligned 
rectangles within the unit cube $[0,1]^d$, i.e., $$H = \lp\{h |
h = \bigcup_{i=1}^k R_i \text{ where } \{R_i\}_{i=1}^k \subset 
[0,1]^d \text{ are disjoint axis-aligned rectangles over } [0,1]^d \rp\}.
$$
Let $h_1, h_2$ be two unknown hypotheses from $H$.
Given $\eps > 0$ and sample access to $(x, h_i(x))$ where $x$ follows the uniform distribution over $[0,1]^d$, there exists an efficient algorithm which distinguishes between (i) $h_1(x) = h_2(x)$ for all $x$ and (ii)
$ \E_{ x \sim U } \lp[ \mathbbm 1 \{ h_1(x) \neq h_2(x) \} \rp] > \eps $ where $U$ is uniform distribution over $[0,1]^d$. Moreover, the algorithm has sample complexity
$
C \; k^{6/7} \; \eps^{ -2 \alpha_d / 3 } \; \log^d(k) \; 2^{d/3}
$, 
where $C$ is a sufficiently large constant and $\alpha_d = O(d^2 2^{2^{d+1}})$.
\end{corollary}
\begin{proof}
Consider the distributions $\p, \q$ defined as follow. 
To take a sample from $\p$, we take a sample $(x, h_1(x))$ where $x \sim U$.
If $h_1(x) = 1$, we return $x$. Otherwise, we return some arbitrarily chosen point $s \not \in [0, 1]^d$.
We define $\q$ similarly based on $h_2$.
If $h_1$ and $h_2$ are identical, it is easy to see that $\p = \q$.
If $\E_{ x \sim U } \lp[ \mathbbm 1 \{ h_1(x) \neq h_2(x) \} \rp]$, we claim $ \snorm{\Ak}{\p- \q} \geq \eps/2 $.
Suppose $h_1$ is the union of the rectangles $\{R_i\}_{i=1}^k$ and $h_2$ is the union of the rectangles $\{R_i'\}_{i=1}^k$.
Then we have
\begin{align*}
&\E_{ x \sim U } \lp[ \mathbbm 1 \{ h_1(x) \neq h_2(x) \} \rp] \\
&= \int_{x \in [0,1]^d} U(x) \; \mathbbm 1 \lp\{ x \in \bigcup_{i=1}^k R_i  \backslash \bigcup_{i=1}^k R_i' \rp\} 
+ \int_{x \in [0,1]^d} U(x) \; \mathbbm 1 \lp\{ x \in \bigcup_{i=1}^k R_i'  \backslash \bigcup_{i=1}^k R_i \rp\} 
\\
&\leq 2 \max \lp( 
\sum_{i=1}^k \int_{x \in [0,1]^d} U(x) \; \mathbbm 1 \lp\{ x \in R_i \backslash \bigcup_{i=1}^k R_i' \rp\} \, , \, 
\sum_{i=1}^k \int_{x \in [0,1]^d} U(x) \; \mathbbm 1 \lp\{ x \in R_i' \backslash \bigcup_{i=1}^k R_i \rp\}
\rp).
\end{align*}
Without loss of generality, we assume the first term is larger. Then, we have
\begin{align*}
\sum_{i=1}^k \int_{x \in [0,1]^d} U(x) \; \mathbbm 1 \lp\{ x \in R_i \backslash \bigcup_{i=1}^k R_i' \rp\}
\geq \frac{1}{2} \eps.
\end{align*}
if $\E_{ x \sim U } \lp[ \mathbbm 1 \{ h_1(x) \neq h_2(x) \} \rp] > \eps$.
On the other hand, 
we also have
\begin{align*}
\sum_{i=1}^k \int_{x \in [0,1]^d} U(x) \; \mathbbm 1 \lp\{ x \in R_i \backslash \bigcup_{i=1}^k R_i' \rp\}
=
\sum_{i=1}^k \p(R_i) - \q(R_i).
\end{align*}
Thus, this gives $\snorm{\Ak}{\p - \q} \geq \eps/2$.
Therefore, we can essentially distinguish between the two cases by performing $\Ak$ closeness testing between $\p, \q$ with accuracy parameter $\eps/2$.
\end{proof}

 
